$\mathtt{DistP}$: Scaling Local-Update Training with Zero-Shot Hyperparameter Transfer

Local-update methods offer a communication-efficient alternative to Distributed Data Parallelism ($\mathtt{DDP}$), but introduce additional hyperparameters that require costly tuning. For $\mathtt{DDP}$, zero-shot hyperparameter transfer reduces this cost by reusing settings tuned on smaller models, but its applicability to local-update training remains unclear. We propose $\mathtt{DistP}$, a theoretical framework extending existing transfer rules from $\mathtt{DDP}$ to local-update training with varying worker counts, local steps, and outer optimizers. With averaging as the outer optimizer, $\mathtt{DistP}$ supports learning-rate transfer across width and depth while improving model quality. The tuned inner learning rate also directly transfers across synchronization intervals, but follows two regimes when increasing the global batch size: square-root learning-rate scaling for larger local batches and a fixed reference rate for additional workers. We then generalize width and depth transfer to other outer optimizers, enabling stable scaling with $\mathtt{Adam}$. However, with momentum in the outer optimizer, changing batch size or local steps can require inner--outer learning-rate tuning, consistent with prior work. In language-modeling experiments at $823$M parameters, $\mathtt{DistP}$ reduces validation loss by $8.1\%$ and improves mean downstream accuracy by $10\%$ relative to baselines without retuning at the larger scale. Fitted scaling laws suggest that this advantage grows with the compute budget, reinforcing the benefits of $\mathtt{DistP}$ for communication-efficient training.

==> preamble/adapter.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\makeatletter

%
\def\@paper@title{Untitled}
\let\@paper@titlerunning\@empty
\let\@paper@keywords\@empty
\let\@paper@code\@empty
\let\@paper@plainauthors\@empty
\let\@paper@displayauthors\@empty
\let\@paper@displayaffils\@empty
\let\@paper@corrdisplay\@empty
\let\@paper@titlelogo\@empty
\def\paper@titlelogoheight{3.0em}
\def\paper@abstractfile{sections/abstract}
\newcounter{paper@affil}
\let\@neurips@authors\@empty
\let\@neurips@affils\@empty
\let\@neurips@corr\@empty
\let\@mlsys@authors\@empty
\let\@mlsys@affils\@empty
\let\@mlsys@corr\@empty
\newif\if@paper@firstauthor \@paper@firstauthortrue
\newif\if@paper@firstdisplayauthor \@paper@firstdisplayauthortrue
\newif\if@paper@hasequal \@paper@hasequalfalse
\newlength{\paper@titlecardinnerwidth}

\def\paper@titlecardpadding{0.30cm}
\def\paper@titlecardradius{10pt}

\definecolor{paperBrandCamlsysBlue}{HTML}{102344}
\definecolor{paperBrandCambridgeRed}{HTML}{EF2E31}
\definecolor{paperBrandCambridgeGold}{HTML}{FDDD04}
\colorlet{paperTitleBgCamlsys}{paperBrandCamlsysBlue!8!white}
\colorlet{paperTitleBgCambridgeGold}{paperBrandCambridgeGold!8!white}
\colorlet{paperTitleBgCambridge}{paperBrandCambridgeRed!3!paperTitleBgCambridgeGold}
\colorlet{paperTitleBgNeutral}{black!2!white}
\colorlet{paperTitleBg}{paperTitleBgCamlsys}
\definecolor{paperTitleFg}{HTML}{1F2328}
\definecolor{paperTitleMuted}{HTML}{4D5560}
\def\paper@titlebg@camlsys{camlsys}
\def\paper@titlebg@cambridge{cambridge}
\def\paper@titlebg@neutral{neutral}

%
\csdef{paper@sym@equal}{*}

%
\newcommand{\paperTitle}[1]{\def\@paper@title{#1}}
\newcommand{\paperKeywords}[1]{\def\@paper@keywords{#1}}
\newcommand{\paperCode}[1]{\def\@paper@code{#1}}
\newcommand{\paperAbstractFile}[1]{\def\paper@abstractfile{#1}}
\newcommand{\paperTitleLogo}[1]{\def\@paper@titlelogo{#1}}
\newcommand{\paperTitleLogoHeight}[1]{\def\paper@titlelogoheight{#1}}
\newcommand{\paperTitleBackground}[1]{%
  \edef\paper@titlebg@choice{#1}%
  \ifx\paper@titlebg@choice\paper@titlebg@camlsys
    \colorlet{paperTitleBg}{paperTitleBgCamlsys}%
  \else
    \ifx\paper@titlebg@choice\paper@titlebg@cambridge
      \colorlet{paperTitleBg}{paperTitleBgCambridge}%
    \else
      \ifx\paper@titlebg@choice\paper@titlebg@neutral
        \colorlet{paperTitleBg}{paperTitleBgNeutral}%
      \else
        \ClassWarning{paper}{Unknown title-card background theme `\paper@titlebg@choice'; keeping current theme}%
      \fi
    \fi
  \fi
}
\paperTitleBackground{\paper@titlebg}
\newcommand{\paperTitleRunning}[1]{%
  \def\@paper@titlerunning{#1}%
  \ifpaper@mlsys \mlsystitlerunning{#1}\fi  %
}

%
%
\newcommand{\addAffiliation}[2]{%
  \stepcounter{paper@affil}%
  \csedef{paper@affil@#1}{\thepaper@affil}%
  \ifnum\value{paper@affil}>\@ne \appto\@paper@displayaffils{\quad}\fi
  \protected@eappto\@paper@displayaffils{\noexpand\textsuperscript{\arabic{paper@affil}}}%
  \appto\@paper@displayaffils{#2}%
  \ifpaper@neurips
    \ifnum\value{paper@affil}>\@ne \appto\@neurips@affils{\quad}\fi
    \protected@eappto\@neurips@affils{\noexpand\textsuperscript{\arabic{paper@affil}}}%
    \appto\@neurips@affils{#2}%
  \fi
  \ifpaper@mlsys
    \appto\@mlsys@affils{\mlsysaffiliation{#1}{#2}}%
  \fi
}

%
%
\newcommand{\paper@resolvekey}[1]{%
  \ifcsdef{paper@sym@#1}{%
    \ifstrequal{#1}{equal}{\@paper@hasequaltrue}{}%
    \protected@eappto\@paper@syms{\csuse{paper@sym@#1}}%
  }{%
    \ifcsdef{paper@affil@#1}{%
      \ifx\@paper@nums\@empty\else\appto\@paper@nums{,}\fi
      \protected@eappto\@paper@nums{\csuse{paper@affil@#1}}%
    }{\ClassWarning{paper}{\noexpand\addAuthor: unknown key `#1'}}%
  }%
}
%
\newcommand{\addAuthor}[2]{%
  \ifx\@paper@plainauthors\@empty
    \appto\@paper@plainauthors{#1}%
  \else
    \appto\@paper@plainauthors{, #1}%
  \fi
  \let\@paper@nums\@empty \let\@paper@syms\@empty
  \forcsvlist{\paper@resolvekey}{#2}%
  \if@paper@firstdisplayauthor\else\appto\@paper@displayauthors{,\space}\fi
  %
  \protected@eappto\@paper@displayauthors{%
    \noexpand\mbox{\unexpanded{#1}\noexpand\textsuperscript{\@paper@nums\@paper@syms}}}%
  \@paper@firstdisplayauthorfalse
  \ifpaper@neurips
    \if@paper@firstauthor\else\appto\@neurips@authors{,\space}\fi
    \appto\@neurips@authors{#1}%
    \protected@eappto\@neurips@authors{\noexpand\textsuperscript{\@paper@nums\@paper@syms}}%
    \@paper@firstauthorfalse
  \fi
  \ifpaper@mlsys
    \appto\@mlsys@authors{\mlsysauthor{#1}{#2}}%
  \fi
}

%
\newcommand{\correspondingAuthor}[2]{%
  \appto\@paper@corrdisplay{\mbox{#1 \texttt{<#2>}}}%
  \ifpaper@neurips \appto\@neurips@corr{\thanks{Correspondence to: #1 \texttt{<#2>}}}\fi
  \ifpaper@mlsys   \appto\@mlsys@corr{\mlsyscorrespondingauthor{#1}{#2}}\fi
}

%
%
\newcommand{\paper@setneuripspdfauthor}{%
  \hypersetup{pdfauthor={\@paper@plainauthors}}%
}
\newcommand{\paper@setmlsyspdfauthor}{%
  \hypersetup{pdfauthor={\@paper@plainauthors}}%
}
\newcommand{\paper@setpdfmetadata}{%
  \@ifpackageloaded{hyperref}{%
    \hypersetup{pdftitle={\@paper@title}}%
    \ifx\@paper@keywords\@empty\else
      \hypersetup{pdfkeywords={\@paper@keywords}}%
    \fi
    \ifpaper@neurips
      \paper@setneuripspdfauthor
    \fi
    \ifpaper@mlsys
      \paper@setmlsyspdfauthor
    \fi
  }{}%
}

%
\newcommand{\paper@titleLogoGraphic}{%
  \IfFileExists{\@paper@titlelogo}{%
    \includegraphics[height=\paper@titlelogoheight,width=\linewidth,keepaspectratio]{\@paper@titlelogo}%
  }{%
    \ClassWarning{paper}{Title logo `\@paper@titlelogo' not found}%
    \fbox{\rule{0pt}{\paper@titlelogoheight}\textsf{\small logo}}%
  }%
}

\newcommand{\paperTitleFont}{\huge}
\newcommand{\paper@titleLine}{%
  \ifx\@paper@titlelogo\@empty
    {\RaggedRight\hyphenpenalty=10000\exhyphenpenalty=10000\sffamily\bfseries\paperTitleFont\color{paperTitleFg}\@paper@title\par}%
  \else
    \noindent
    \begin{minipage}[c]{0.075\linewidth}
      \centering\paper@titleLogoGraphic
    \end{minipage}\hspace{0.015\linewidth}%
    \begin{minipage}[c]{0.91\linewidth}
      {\RaggedRight\hyphenpenalty=10000\exhyphenpenalty=10000\sffamily\bfseries\paperTitleFont\color{paperTitleFg}\@paper@title\par}%
    \end{minipage}\par
  \fi
}

\newcommand{\paper@identityBlock}{%
  \ifx\@paper@displayauthors\@empty\else
    {\sffamily\bfseries
      \ifpaper@neurips\fontsize{9.5pt}{12pt}\else\fontsize{10.5pt}{13pt}\fi
      \selectfont\raggedright
      \color{paperTitleFg}\@paper@displayauthors\par}%
  \fi
  \ifx\@paper@displayaffils\@empty\else
    \vspace{0.10cm}%
    {\small\raggedright\color{paperTitleMuted}\@paper@displayaffils\par}%
  \fi
}

\newcommand{\paper@metadataText}{%
  \if@paper@hasequal
    \textsuperscript{*}Equal contribution.\par
  \fi
  \ifx\@paper@corrdisplay\@empty\else
    {\sffamily\bfseries Correspondence:} \@paper@corrdisplay\par
  \fi
  \ifx\@paper@keywords\@empty\else
    {\sffamily\bfseries Keywords:} \@paper@keywords\par
  \fi
  \ifx\@paper@code\@empty\else
    {\sffamily\bfseries Code:} \@paper@code\par
  \fi
}

\newsavebox{\paper@logobox}
\newcommand{\paper@metadataRow}{%
  \ifx\paper@logos\paper@logos@none
    {\small\raggedright\color{paperTitleMuted}\paper@metadataText\par}%
  \else
    \sbox{\paper@logobox}{\paperLogoStrip}%
    \noindent
    \begin{minipage}[c]{\dimexpr\linewidth-\wd\paper@logobox-1em\relax}
      {\small\raggedright\color{paperTitleMuted}\paper@metadataText\par}%
    \end{minipage}\hfill
    \usebox{\paper@logobox}\par
  \fi
}

\newcommand{\paper@titlecard}{%
  \begingroup
    \setlength{\paper@titlecardinnerwidth}{\dimexpr\linewidth-\paper@titlecardpadding-\paper@titlecardpadding\relax}%
    \noindent
    \begin{tikzpicture}
      \node[
        fill=paperTitleBg,
        rounded corners=\paper@titlecardradius,
        inner sep=\paper@titlecardpadding,
        outer sep=0pt,
        text width=\paper@titlecardinnerwidth,
        align=left
      ] (paperTitleCardNode) {%
        \begin{minipage}{\paper@titlecardinnerwidth}
          \setlength{\parindent}{0pt}%
          \setlength{\parskip}{0pt}%
          \raggedright
          \paper@titleLine
          \vspace{0.16cm}%
          \paper@identityBlock
          \vspace{0.20cm}%
          {\small\justifying\color{paperTitleFg}{\sffamily\bfseries Abstract.}\space\input{\paper@abstractfile}\par}%
          \vspace{0.22cm}%
          \paper@metadataRow
        \end{minipage}%
      };%
    \end{tikzpicture}%
    \par\vspace{0.10cm}%
  \endgroup
}

\newcommand{\paper@setmlsysrunninghead}{%
  \ifx\@paper@titlerunning\@empty
    \gdef\@mlsystitlerunning{\@paper@title}%
  \else
    \gdef\@mlsystitlerunning{\@paper@titlerunning}%
  \fi
  \chead{\small\bf\@mlsystitlerunning}%
  \thispagestyle{empty}%
}

\newcommand{\paper@mlsysNotice}{%
  \begingroup
    \let\thefootnote\relax
    %
    \let\@footnotetext\H@@footnotetext
    \footnotetext{\hspace*{-\footnotesep}\Notice@String}%
  \endgroup
}

%
\newcommand{\makepapertitle}{%
  \paper@setpdfmetadata
  \ifpaper@neurips
    \par
    \begingroup
      \thispagestyle{empty}%
      \paper@titlecard
      \@notice
    \endgroup
  \fi
  \ifpaper@mlsys
    \paper@setmlsysrunninghead
    \twocolumn[%
      \paper@titlecard
      \vskip 0.06in
    ]%
    \paper@mlsysNotice
  \fi
}

\makeatother


==> preamble/format.tex <==
%
%
%
%
\makeatletter
%
\PassOptionsToPackage{numbers,sort&compress}{natbib}

\newif\ifpaper@neurips
\newif\ifpaper@mlsys
\newif\ifpaper@twocolumn

\def\paper@@neurips{neurips}
\def\paper@@mlsys{mlsys}
\ifx\paper@format\paper@@mlsys
  \paper@mlsystrue
\else
  \ifx\paper@format\paper@@neurips
    \paper@neuripstrue
  \else
    \ClassError{paper}{Unknown format `\paper@format'; use format=neurips or format=mlsys}{}%
  \fi
\fi

%
\ifpaper@neurips
  \paper@twocolumnfalse
  \RequirePackage[preprint]{neurips_2026}%
  %
  \AtBeginDocument{%
    \raggedbottom
    \setcounter{topnumber}{3}%
    \setcounter{bottomnumber}{2}%
    \setcounter{totalnumber}{5}%
    \renewcommand{\topfraction}{.9}%
    \renewcommand{\bottomfraction}{.9}%
    \renewcommand{\textfraction}{.08}%
    \renewcommand{\floatpagefraction}{.75}%
    \setlength{\floatsep}{8pt plus 2pt minus 2pt}%
    \setlength{\textfloatsep}{10pt plus 2pt minus 2pt}%
    \setlength{\intextsep}{10pt plus 2pt minus 2pt}%
  }%
  \def\paperbibstyle{unsrtnat}%
\fi

%
\ifpaper@mlsys
  \paper@twocolumntrue
  %
  \providecommand{\theHalgorithm}{\arabic{algorithm}}%
  \RequirePackage[accepted]{mlsys2026}%
  %
  \AtBeginDocument{%
    \raggedbottom
    \setcounter{topnumber}{3}%
    \setcounter{totalnumber}{5}%
    \setcounter{dbltopnumber}{3}%
    \renewcommand{\topfraction}{.9}%
    \renewcommand{\dbltopfraction}{.9}%
    \renewcommand{\textfraction}{.08}%
    \renewcommand{\floatpagefraction}{.75}%
    \renewcommand{\dblfloatpagefraction}{.75}%
    \setlength{\floatsep}{8pt plus 2pt minus 2pt}%
    \setlength{\textfloatsep}{10pt plus 2pt minus 2pt}%
    \setlength{\dblfloatsep}{8pt plus 2pt minus 2pt}%
    \setlength{\dbltextfloatsep}{10pt plus 2pt minus 2pt}%
  }%
  \def\paperbibstyle{unsrtnat}%
\fi

%
%
\AtBeginDocument{%
  \setlength{\@fptop}{0pt}%
  \setlength{\@fpsep}{10pt}%
  \setlength{\@fpbot}{0pt plus 1fil}%
  \setlength{\@dblfptop}{0pt}%
  \setlength{\@dblfpsep}{10pt}%
  \setlength{\@dblfpbot}{0pt plus 1fil}%
}%

%
\setcitestyle{numbers,square,comma}
\makeatother


==> preamble/logos.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
\makeatletter

\newcommand{\paper@logoheight}{13mm}

%
\newcommand{\paper@logo}[2]{%
  \raisebox{-0.5\height}{%
    \IfFileExists{branding/#1.pdf}{\includegraphics[height=\paper@logoheight]{branding/#1.pdf}}{%
    \IfFileExists{branding/#1.png}{\includegraphics[height=\paper@logoheight]{branding/#1.png}}{%
    \IfFileExists{branding/#1.jpg}{\includegraphics[height=\paper@logoheight]{branding/#1.jpg}}{%
    \fbox{\rule[-2.5mm]{0pt}{\paper@logoheight}\textsf{\small\,#2\,}}}}}%
  }%
}

%
%
\newcommand{\paper@logoOr}[3]{%
  \IfFileExists{branding/#1.pdf}{\paper@logo{#1}{#3}}{%
  \IfFileExists{branding/#1.png}{\paper@logo{#1}{#3}}{%
  \IfFileExists{branding/#1.jpg}{\paper@logo{#1}{#3}}{%
  \paper@logo{#2}{#3}}}}%
}

\def\paper@logos@none{none}
\def\paper@logos@cc{camlsys-cambridge}
\def\paper@logos@ccf{camlsys-cambridge-flower}
\def\paper@logos@ccfz{camlsys-cambridge-flower-zib}
\def\paper@logos@ccfzc{camlsys-cambridge-flower-zib-cnrs}
\def\paper@logos@ccfzcs{camlsys-cambridge-flower-zib-cnrs-sofair}

\newcommand{\paperLogoStrip}{%
  \ifx\paper@logos\paper@logos@none\else
    \begingroup
      \renewcommand{\paper@logoheight}{9mm}%
      \ifx\paper@logos\paper@logos@ccfzc
        \renewcommand{\paper@logoheight}{8mm}%
      \fi
      \ifx\paper@logos\paper@logos@ccfzcs
        \renewcommand{\paper@logoheight}{8mm}%
      \fi
      \paper@logoOr{camlsys}{big_camlsys_logo}{CaMLSys}\hspace{0.4em}%
      \paper@logo{cambridge}{University of Cambridge}%
      \ifx\paper@logos\paper@logos@ccf
        \hspace{0.55em}\paper@logo{flower}{Flower Labs}%
      \fi
      \ifx\paper@logos\paper@logos@ccfz
        \hspace{0.55em}\paper@logo{flower}{Flower Labs}%
        \hspace{0.55em}{\renewcommand{\paper@logoheight}{7mm}%
          \paper@logo{zib}{Zuse Institute Berlin}}%
      \fi
      \ifx\paper@logos\paper@logos@ccfzc
        \hspace{0.4em}\paper@logo{flower}{Flower Labs}%
        \hspace{0.4em}{\renewcommand{\paper@logoheight}{7mm}%
          \paper@logo{zib}{Zuse Institute Berlin}}%
        \hspace{3.5mm}{\renewcommand{\paper@logoheight}{7mm}%
          \paper@logo{cnrs}{CNRS}}%
      \fi
      \ifx\paper@logos\paper@logos@ccfzcs
        \hspace{2mm}{\renewcommand{\paper@logoheight}{5mm}%
          \paper@logo{sofair}{SOFAIR}}%
        \hspace{2mm}{\renewcommand{\paper@logoheight}{7mm}%
          \paper@logo{zib}{Zuse Institute Berlin}}%
        \hspace{0.4em}{\renewcommand{\paper@logoheight}{7mm}%
          \paper@logo{cnrs}{CNRS}}%
        \hspace{0.4em}\paper@logo{flower}{Flower Labs}%
      \fi
    \endgroup
  \fi
}

\newcommand{\logoHeader}{%
  \ifx\paper@logos\paper@logos@none\else
    \begin{center}%
      \noindent\begin{minipage}{\textwidth}\centering
        \paperLogoStrip
      \end{minipage}%
    \end{center}%
    \vspace{0.5\baselineskip}%
  \fi
}

\makeatother


==> preamble/macros.tex <==
%
%
\makeatletter

%
\graphicspath{{figures/}{figures/plots/}{figures/diagrams/}{figures/tikz/}{branding/}}

%
%
\input{preamble/scaling-colours}
\newcommand{\widthaxis}[1]{\textcolor{ScaleWidth}{#1}}
\newcommand{\depthaxis}[1]{\textcolor{ScaleDepth}{#1}}
\newcommand{\batchaxis}[1]{\textcolor{ScaleBatch}{#1}}
\newcommand{\dataaxis}[1]{\textcolor{ScaleTokens}{#1}}
\newcommand{\distaxis}[1]{\textcolor{ScaleDistributed}{#1}}

%
%
%
%
\newenvironment{widefigure}[1][tbp]
  {\ifpaper@twocolumn \@nameuse{figure*}[#1]\else \@nameuse{figure}[#1]\fi}
  {\ifpaper@twocolumn \@nameuse{endfigure*}\else \@nameuse{endfigure}\fi}
\newenvironment{widetable}[1][tbp]
  {\ifpaper@twocolumn \@nameuse{table*}[#1]\else \@nameuse{table}[#1]\fi}
  {\ifpaper@twocolumn \@nameuse{endtable*}\else \@nameuse{endtable}\fi}

%
\renewcommand{\thesubfigure}{(\alph{subfigure})}
\captionsetup[subfigure]{labelformat=simple}
\newcommand{\rqleftfraction}{.5268}
\newcommand{\rqrightfraction}{.4532}
\newcommand{\rqsplitpanels}[4][.74]{%
  \begin{minipage}{\linewidth}\centering
  \includegraphics[width=#1\linewidth]{figures/plots/rq1-prenorm/rq1-#4-legend.pdf}\par\nointerlineskip
  \begin{subfigure}[t]{\rqleftfraction\linewidth}
    \centering
    \captionsetup{position=top,skip=3pt}
    \caption{\standardp}\label{#3-sp}
    \includegraphics[width=\linewidth,clip]{figures/plots/rq1-prenorm/#2-sp.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{\rqrightfraction\linewidth}
    \centering
    \captionsetup{position=top,skip=3pt}
    \caption{\method}\label{#3-distp}
    \includegraphics[width=\linewidth,clip]{figures/plots/rq1-prenorm/#2-distp.pdf}
  \end{subfigure}%
  \par\vspace{1pt}\(\eta\)%
  \end{minipage}%
}
%
\newlength{\rqmatrixwidth}
\newcommand{\rqmatrixrow}[4]{%
  \ifnum#4=0\relax
    \makebox[\linewidth][l]{\makebox[\rqmatrixwidth][c]{\small\strut #3}}\par
  \else{\small\strut}\par\fi
  \vspace{2pt}%
  \includegraphics[width=\linewidth]{figures/plots/rq1-prenorm/rq1-#1-row-#2.pdf}\par
}
\newcommand{\rqmatrixpanels}[3]{%
  \begingroup\setlength{\parskip}{0pt}%
  \setlength{\rqmatrixwidth}{\linewidth}%
  \includegraphics[width=.74\linewidth]{figures/plots/rq1-prenorm/rq1-#1-legend.pdf}\par\nointerlineskip
  \begin{subfigure}[t]{\rqleftfraction\linewidth}\centering
    \captionsetup{position=top,skip=3pt}\caption{\standardp}\label{#2-sp}
    \ifnum#3=1\relax\rqmatrixrow{#1}{averaging-sp}{Averaging}{0}\fi
    \rqmatrixrow{#1}{nesterov-sp}{\nesterov}{0}
    \rqmatrixrow{#1}{adam-sp}{\adam}{0}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{\rqrightfraction\linewidth}\centering
    \captionsetup{position=top,skip=3pt}\caption{\method}\label{#2-distp}
    \ifnum#3=1\relax\rqmatrixrow{#1}{averaging-distp}{Averaging}{1}\fi
    \rqmatrixrow{#1}{nesterov-distp}{\nesterov}{1}
    \rqmatrixrow{#1}{adam-distp}{\adam}{1}
  \end{subfigure}\par\vspace{1pt}\(\eta\)%
  \endgroup
}
\newcommand{\rqcadenceheading}{Outer learning rate transfer}
\newcommand{\rqregimepanels}[4]{%
  \begin{subfigure}[t]{.3599\linewidth}\centering
    \captionsetup{position=top,skip=3pt}\caption{Workers \(M/M_0\)}\label{#2}
    \includegraphics[width=\linewidth,clip]{figures/plots/rq23-prenorm/#1-workers.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.2909\linewidth}\centering
    \captionsetup{position=top,skip=3pt}\caption{Local batch \(b/b_0\)}\label{#3}
    \includegraphics[width=\linewidth,clip]{figures/plots/rq23-prenorm/#1-local-batch.pdf}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.3292\linewidth}\centering
    \captionsetup{position=top,skip=3pt}\caption{\rqcadenceheading}\label{#4}
    \includegraphics[width=\linewidth,clip]{figures/plots/rq23-prenorm/#1-local-steps.pdf}
  \end{subfigure}%
}

%
\newcommand{\singlecolumnfloatbarrier}{\ifpaper@twocolumn\else\FloatBarrier\fi}

%
\definecolor{CalloutPeach}{rgb}{1.000,0.965,0.920}
\definecolor{CalloutGold}{rgb}{0.696,0.566,0.234}
%
\newlist{takeawayitems}{enumerate}{1}
\setlist[takeawayitems,1]{
  label=\textbf{\arabic*.},
  widest=III,
  labelindent=0pt,
  leftmargin=*,
  labelsep=0.5em,
  align=right,
  itemsep=1pt,
  parsep=0pt,
  topsep=2pt,
  partopsep=0pt,
  listparindent=0pt
}

\NewDocumentCommand{\introtakeawaybox}{o m}{%
  \begin{tcolorbox}[%
    colback=CalloutPeach,
    colframe=CalloutGold,
    boxrule=0.5pt,
    arc=0pt,
    outer arc=0pt,
    left=5pt,
    right=5pt,
    top=2pt,
    bottom=2pt,
    fontupper={\fontsize{9pt}{11pt}\selectfont\RaggedRight}
  ]
    \IfNoValueTF{#1}{#2}{\textbf{Contributions #1:} #2}%
  \end{tcolorbox}%
  \vspace*{-0.1cm}
}

\NewDocumentCommand{\takeawaybox}{o m}{%
  \begin{tcolorbox}[
    colback=CalloutPeach,
    colframe=CalloutGold,
    boxrule=0.5pt,
    arc=0pt,
    outer arc=0pt,
    left=5pt,
    right=5pt,
    top=2pt,
    bottom=2pt,
    fontupper={\fontsize{9pt}{11pt}\selectfont\RaggedRight}
  ]
    \IfNoValueTF{#1}{\textbf{Takeaway:} #2}{\textbf{#1} #2}%
  \end{tcolorbox}%
  \vspace*{-0.1cm}
}

\makeatother
\newcommand{\dilocofit}{{\upshape\texttt{DiLoCo-fit}}\xspace}
\newcommand{\lordo}{{\upshape\texttt{LoRDO}}\xspace}
\newcommand{\method}{\texorpdfstring{{\upshape\texttt{DistP}}}{DistP}\xspace}
\newcommand{\smallmodel}{{\upshape\texttt{Small}}\xspace}
\newcommand{\mediummodel}{{\upshape\texttt{Medium}}\xspace}
\newcommand{\largemodel}{{\upshape\texttt{Large}}\xspace}
\newcommand{\mup}{\texorpdfstring{{\upshape\texttt{\(\mu\)P}}}{muP}\xspace}
\newcommand{\completep}{{\upshape\texttt{CompleteP}}\xspace}
\newcommand{\completedp}{\texorpdfstring{{\upshape\texttt{Complete\textsuperscript{(d)}P}}}{Complete(d)P}\xspace}
\newcommand{\adam}{{\upshape\texttt{Adam}}\xspace}
\newcommand{\adamw}{{\upshape\texttt{AdamW}}\xspace}
\newcommand{\muon}{{\upshape\texttt{Muon}}\xspace}
\newcommand{\muloco}{{\upshape\texttt{MuLoCo}}\xspace}
\newcommand{\standardp}{{\upshape\texttt{SP}}\xspace}
\newcommand{\ddp}{{\upshape\texttt{DDP}}\xspace}
\newcommand{\sgd}{{\upshape\texttt{SGD}}\xspace}

\newcommand{\diloco}{{\upshape\texttt{DiLoCo}}\xspace}
\newcommand{\localsgd}{{\upshape\texttt{Local SGD}}\xspace}
\newcommand{\sgdm}{{\upshape\texttt{SGD-M}}\xspace}
\newcommand{\nesterov}{{\upshape\texttt{Nesterov}}\xspace}
\newcommand{\mtdao}{{\upshape\texttt{MT-DAO}}\xspace}
\newcommand{\desloc}{{\upshape\texttt{DES-LOC}}\xspace}

\newcommand{\fedavg}{{\upshape\texttt{FedAvg}}\xspace}

%
\newcommand{\slowmo}{{\upshape\texttt{SlowMo}}\xspace}
\newcommand{\fedopt}{{\upshape\texttt{FedOpt}}\xspace}
\newcommand{\photon}{{\upshape\texttt{Photon}}\xspace}
\newcommand{\sparseloco}{{\upshape\texttt{SparseLoCo}}\xspace}
\newcommand{\asyncmesh}{{\upshape\texttt{AsyncMesh}}\xspace}
\newcommand{\fomoe}{{\upshape\texttt{FoMoE}}\xspace}
\newcommand{\zclip}{{\upshape\texttt{ZClip}}\xspace}
\newcommand{\streamingdiloco}{{\upshape\texttt{Streaming DiLoCo}}\xspace}
\newcommand{\asyncdiloco}{{\upshape\texttt{Asynchronous DiLoCo}}\xspace}
\newcommand{\decoupleddiloco}{{\upshape\texttt{Decoupled DiLoCo}}\xspace}
\newcommand{\factoredgossipdiloco}{{\upshape\texttt{Factored Gossip DiLoCo}}\xspace}


==> preamble/microtype-compat.tex <==
% Backport the microtype v3.2b showhyphens fix for older Overleaf installations.
% The 2025-06-01 LaTeX kernel changed this diagnostic command; patch its colour
% group instead of checking/replacing its entire definition. Font expansion
% remains enabled in the paper and is disabled only inside showhyphens.
% Adapted from R Schlicht's microtype (LPPL 1.3c or later), issues #53/#55:
% https://github.com/schlcht/microtype/issues/53
% Loaded from packages.tex with @ already a letter.
\newif\ifpaper@oldmicrotype
\@ifpackagelater{microtype}{2025/05/05}
  {\paper@oldmicrotypefalse}{\paper@oldmicrotypetrue}
\ifPDFTeX
  \ifpaper@oldmicrotype
    % Consume the old check/redefinition pair and patch the current command.
    \long\def\paper@patchshowhyphens[1]#1\DeclareRobustCommand\showhyphens[1]#2{%
      \expandafter\patchcmd\csname showhyphens \endcsname
        {\color@begingroup}{\color@begingroup\pdfadjustspacing\z@}
        {}{\PackageError{paper}{Could not patch showhyphens}{Update microtype to v3.2b or later.}}%
    }
    \patchcmd{\MT@setup@expansion}
      {\MT@exp@cs\CheckCommand{showhyphens }}
      {\paper@patchshowhyphens}
      {}{\PackageError{paper}{Could not apply microtype compatibility fix}{Update microtype to v3.2b or later.}}%
  \fi
\fi


==> preamble/packages.tex <==
%
%
%
\makeatletter

\RequirePackage{etoolbox}   %

%
\RequirePackage{iftex}
\ifPDFTeX
  \RequirePackage[utf8]{inputenc}
  \RequirePackage[T1]{fontenc}
\fi

\RequirePackage{graphicx}
\RequirePackage{booktabs}        %
\RequirePackage{amsmath}
\RequirePackage{amssymb}
%
\DeclareMathSizes{9.5}{9}{7}{5}
\DeclareMathSizes{10.5}{10}{7}{5}
\RequirePackage{mathtools}
\RequirePackage{microtype}
\input{preamble/microtype-compat}
\RequirePackage{ragged2e}       %
\RequirePackage{xurl}           %
%
\AtBeginDocument{%
  \apptocmd{\thebibliography}
    {\RaggedRight\setlength{\parfillskip}{0pt plus 1fil}%
     \finalhyphendemerits=1000000\relax}{}
    {\PackageWarning{paper}{Could not set bibliography final-line spacing}}%
}
\RequirePackage{xcolor}
\RequirePackage{colortbl}        %
\RequirePackage{xparse}
\RequirePackage{xspace}
\RequirePackage{enumitem}
\RequirePackage{tikz}
\usetikzlibrary{arrows.meta,positioning,shapes.geometric,calc,fit,backgrounds,decorations.pathreplacing}
%
\let\paper@native@makecaption\@makecaption
\RequirePackage{subcaption}
\AtBeginDocument{\let\@makecaption\paper@native@makecaption}
\captionsetup[subfigure]{font=small,skip=2pt,labelformat=parens,
  justification=centering,hypcap=true}
\RequirePackage{placeins}        %
\RequirePackage{needspace}       %
\RequirePackage{etoc}            %

%
%
\@ifpackageloaded{hyperref}{}{\RequirePackage{hyperref}}
\definecolor{ThemeBlue}{rgb}{0.10,0.20,0.55}
\definecolor{ThemeNavy}{HTML}{102344}
\definecolor{ThemeGray}{HTML}{4D5560}
\hypersetup{
  linkcolor=ThemeNavy,
  urlcolor=ThemeBlue,
  citecolor=ThemeBlue,
  filecolor=ThemeGray,
  colorlinks=true,
  breaklinks=true,
  bookmarksopen=true
}
\RequirePackage[capitalise, nameinlink]{cleveref}
\RequirePackage{tcolorbox}


\RequirePackage{sourcecodepro}

\makeatother


==> preamble/scaling-colours.tex <==
%
\definecolor{ScaleWidth}{HTML}{332288}
\definecolor{ScaleDepth}{HTML}{117733}
\definecolor{ScaleBatch}{HTML}{882255}
\definecolor{ScaleTokens}{HTML}{AA4499}
\definecolor{ScaleDistributed}{HTML}{333333}
%
\providecolor{ThemeNavy}{HTML}{102344}
\providecolor{CalloutPeach}{rgb}{1.000,0.965,0.920}
\providecolor{CalloutGold}{rgb}{0.696,0.566,0.234}


==> sections/abstract.tex <==
Local-update methods offer a communication-efficient alternative to Distributed Data Parallelism~(\ddp), but introduce additional hyperparameters that require costly tuning.
For \ddp, zero-shot hyperparameter transfer reduces this cost by reusing settings tuned on smaller models, but its applicability to local-update training remains unclear.
We propose \method, a theoretical framework extending existing transfer rules from \ddp to local-update training with varying worker counts, local steps, and outer optimizers.
With averaging as the outer optimizer, \method supports learning-rate transfer across width and depth while improving model quality.
The tuned inner learning rate also directly transfers across synchronization intervals, but follows two regimes when increasing the global batch size: square-root learning-rate scaling for larger local batches and a fixed reference rate for additional workers.
We then generalize width and depth transfer to other outer optimizers, enabling stable scaling with \adam. However, with momentum in the outer optimizer, changing batch size or local steps can require inner--outer learning-rate tuning, consistent with prior work.
In language-modeling experiments at $823$M parameters, \method reduces validation loss by $8.1\%$ and improves mean downstream accuracy by $10\%$ relative to baselines without retuning at the larger scale.
Fitted scaling laws suggest that this advantage grows with the compute budget, reinforcing the benefits of \method for
communication-efficient training.

